Optimal performance of a tontine overlay subject to withdrawal constraints

We consider the holder of an individual tontine retirement account, with maximum and minimum withdrawal amounts (per year) specified. The tontine account holder initiates the account at age 65, and earns mortality credits while alive, but forfeits all wealth in the account upon death. The holder desires to maximize total withdrawals, and minimize the expected shortfall, assuming the holder survives to age 95. The investor controls the amount withdrawn each year and the fraction of the investments in stocks and bonds. The optimal controls are determined based on a parametric model fitted to almost a century of market data. The optimal control algorithm is based on dynamic programming and solution of a partial integro differential equation (PIDE) using Fourier methods. The optimal strategy (based on the parametric model) is tested out of sample using stationary block bootstrap resampling of the historical data. In terms of an expected total withdrawal, expected shortfall (EW-ES) efficient frontier, the tontine overlay greatly outperforms an optimal strategy (without the tontine overlay), which in turn outperforms a constant weight strategy with withdrawals based on the ubiquitous four per cent rule.

==> README <==

Subdirectories:
   matlab   data and M-files for matlab plots
    tecplot_plot_data  data for tecplot plots
                           - fraction, wealth, withdrawal percentiles
                           - heat maps
                           - *.dat files have original data
   heat_map_controls - MC_controls.dat file, kappa = .180
-------------------------------------------


 https://www.editorialmanager.com/ime/
 userid: paforsyt@uwaterloo.ca
 passwd: CompassRose1!

Quantitative Finance
   userid: paforsyt@uwaterloo.ca
   passwd: CompassRose2!1
   https://mc.manuscriptcentral.com/rquf
-------------------------------------------

Passwds:
   Appl Math Fin
    userid: paforsyt@uwaterloo.ca
    passwd: Rocket!2718
 http://mc.manuscriptcentral.com/ramf
----------------------------------------
ASTIN Bulletin
     userid: paforsyt@uwaterloo.ca
     passwd: CompassRose12
------------------------------
Annals of Operations Research
   WITHDREW MAY 31/2017

  email: paforsyt@uwaterloo.ca
  userid: paforsyt@uwaterloo.ca
  passswd: CompassRose1!

------------------------------------
 NAAJ login:
        id: paforsyt@uwaterloo.ca
      passwd: CompassRose1!2
----------------------------------

Insurance: Math & Economics

 https://www.editorialmanager.com/ime/
 userid: paforsyt@uwaterloo.ca
 passwd: CompassRose1!

---------------------------------------


------------------------------------

SIFIN
   userid: paforsyt
   passwd: CompassRose1!
     http://sifin.siam.org

-----------------------------------
---------------------------------------

International Journal Theortical and Applied Finance
userid: PeterForsyt
pass:   CompassRose1!




-----------------------------------
To submit Latex files:
 submitted version:
   1) cp paper.bbl paperbbl.tex
   2) remove bibliography statements from paper.tex
   2) replace by
       \input{paperbbl}


--------------------------------------




-------- Forwarded Message --------
Subject: 	Submission to Insurance: Mathematics and Economics - manuscript number
Date: 	29 Aug 2021 16:53:42 -0400
From: 	Insurance: Mathematics and Economics <em@editorialmanager.com>
Reply-To: 	Insurance: Mathematics and Economics <insmathecon@gmail.com>
To: 	Peter Forsyth <paforsyt@uwaterloo.ca>


*This is an automated message.* 

Manuscript Number: IME-D-21-00314
Short Term Decumulation Strategies for Underspending Retirees

Dear Professor Forsyth,

Your above referenced submission has been assigned a manuscript number: IME-D-21-00314.

To track the status of your manuscript, please log in as an author at https://www.editorialmanager.com/ime/, and navigate to the "Submissions Being Processed" folder.

Thank you for submitting your work to this journal.

Kind regards,
Insurance: Mathematics and Economics     

More information and support

You will find information relevant for you as an author on Elsevier’s Author Hub: https://www.elsevier.com/authors

FAQ: How can I reset a forgotten password? https://service.elsevier.com/app/answers/detail/a_id/28452/supporthub/publishing/ For further assistance, please visit our customer service site: https://service.elsevier.com/app/home/supporthub/publishing/
Here you can search for solutions on a range of topics, find answers to frequently asked questions, and learn more about Editorial Manager via interactive tutorials. You can also talk 24/7 to our customer support team by phone and 24/7 by live chat and email

__________________________________________________
In compliance with data protection regulations, you may request that we remove your personal registration details at any time. (Use the following URL: https://www.editorialmanager.com/ime/login.asp?a=r). Please contact the publication office if you have any questions.

